Eco-Routing Using Open Street Maps

A vehicle's fuel consumption depends on its type, the speed, the condition, and the gradients of the road on which it is moving. We developed a Routing Engine for finding an eco-route (one with low fuel consumption) between a source and a destination. Open Street Maps has data on road conditions. We used CGIAR-CSI road elevation data 16[4] to integrate the road gradients into the proposed route-finding algorithm that modifies Open Street Routing Machine (OSRM). It allowed us to dynamically predict a vehicle's velocity, considering both the conditions and the road segment's slope. Using Highway EneRgy Assessment (HERA) methodology, we calculated the fuel consumed by a vehicle given its type and velocity. We have created both web and mobile interfaces through which users can specify Geo coordinates or human-readable addresses of a source and a destination. The user interface graphically displays the route obtained from the proposed Routing Engine with a detailed travel itinerary.

==> sections/Incorrectelevation.tex <==
The road network graph built from OSM by OSRM has edge weights assigned either as distances or as the time to those distances considering the road types.  For computing the least fuel cost path, we need to change the edge weights to fuel consumption parameters using equation~\ref{eq:FC}, which is straightforward. However, in the equation, we still have to incorporate  Road Gradient Factor. But the OSM data set like Google Maps doesn't have those details. So, the elevation needs to be computed only from available data. Let us find a method to determine the road gradient by integrating the elevation data.

\subsection{Integrating Elevation}

The gradient of a road affects the velocity of a vehicle moving on the road. Since speed affects a vehicle's fuel consumption, we need to know the road gradient to be able to estimate the fuel consumption when a vehicle moves either up or down a road gradient. We assign a penalty coefficient to velocity, which varies according to the known gradient of the road. The penalty function is determined based on the time required to cover a distance over flat road versus the time needed to cover the same distance on the road with known elevation either in ascent or in descent. A road elevation has the effect of slowing down the vehicle while moving up or down the gradient. Hence, the estimation of fuel consumption can be made based on the modified velocity of the vehicle.   %Since, the gradient affect velocity, and we can penalize the velocity depends on the gradient. Here first I'll be discussing about the elevation data.\\

Before deciding on a penalty factor, as indicated above, it is important to understand the calculation of the road gradient. %So what we need for calculating the gradient of the road? 
As Fig.~\ref{fig:altitude}~\cite{gradient_wiki} shows the difference in the height difference between the starting and the endpoint of a road segment gives the ascent or descent the given stretch of the road. 
\begin{figure}[htb]
    \centering
    \includegraphics[scale=0.2,angle=-90]{images/gradient.pdf}
    \caption{Gradient of a road segment.}
    \label{fig:altitude}
\end{figure}
Given the altitude and the length (hypotenuse) of the road segment, we can find the elevation. All road gradient measurements are with reference to the sea level. %Which i for any given starting point and ending point, we need to able to tell the height difference. 
If the elevation data is available for every point on the globe, then we can easily calculate the raise or drop in elevation between any two points.
%Therefore, we use the elevation (height above the sea level) data to compute gradient. 

Simply put, Digital Elevation Model (DEM)~\cite{zhang1994digital} is a digital representation of the Earth's topography. In particular, it is 3D Computer Graphics (3D-CG) representation of the land surface generated from the terrain elevation data. DEM is created by collecting elevation from equally or unequally spaced points~\cite{remote_sensing}. The collected elevation information can be used for continuous spatial representation of any terrain. DEM gives elevation information of terrain, including trees, or any human-made structures with reference to Mean Sea Level (MSL).

Depending upon how the elevation information is structured and stored, we can classify DEM into two types:
\begin{enumerate}
  \item Regular square grids,
  \item Triangulated irregular networks (TIN). 
\end{enumerate}
Grid DEM is stored as a raster map with each pixel having the information about the elevation of the terrain. TIN data also includes features like peaks, slopes, conic pits. So, TIN-DEM considered being more accurate for extracting structural information. 
It is possible to obtain elevation information using field surveys from topographic contours, aerial photographs, or satellite imageries using photogrammetric techniques. Photogrammetry is an of three-dimensional measurements from two-dimensional data. Recently radar interferometric techniques and Laser altimetry have also been used to generate a DEM. Today very high-resolution DEMs at the near-global scale are readily available from various sources~\cite{remote_sensing}. 

Some of the sources of global elevation data set are.
\begin{enumerate}
    \item Global 30 Arc-Second Elevation (GTOPO30): GTOPO~\cite{gtopo30} a global digital elevation model (DEM) with a horizontal grid spacing of 30 arc seconds (approximately 1 kilometer). GTOPO30 was derived from several rasters and vector sources of topographic information. GTOPO30, completed in late 1996, was developed over three years through a collaborative effort led by staff at the US Geological Survey’s EROS Data Center (EDC).

    \item NOAA Global Land One-km Base Elevation (GLOBE): GLOBE~\cite{noaa-globe} is an internationally designed, developed, and independently reviewed global DEM, at a latitude-longitude grid spacing of 30 arc seconds (approx. 1km).
    
    \item Shuttle Radar Topography Mission (SRTM): SRTM~\cite{jarvis2008hole} is an international research effort that obtained DEM on a near-global scale to generate the most complete high-resolution digital topographic database of Earth. Using two radar antennas and a single pass, it collected sufficient data to generate a digital elevation model. This 1-arc second global DEM has a spatial resolution of about 30 meters in most areas. Also, it covers most of the world with an absolute vertical height accuracy of 10 meters approximately.
    
    \item ASTER Global Digital Elevation Model: NASA and Japan’s joint operation was the birth of Advanced Spaceborne Thermal Emission and Reflection Radiometer (ASTER)~\cite{paul2004combining}. ASTER data are used to create detailed maps of the surface temperature of land, emissivity, reflectance, and elevation.
    
    \item Lidar DEM: It is an airplane laser system that sends light pulses. It reflects the terrain and the objects on it. LiDAR~\cite{gesch2009analysis} transmits and receives electromagnetic radiation of the near IR band. Unlike photogrammetry, LiDAR data collection is not affected by sun angle. LIDAR precision depends on the three basic elements of the system: GPS, IMU, and Laser.
\end{enumerate}

%{\color{red} Comment: Only SRTM is mentioned, other have not been discussed. It will be better if you discuss why other elevation data are not suitable for our purpose.}

\begin{table*}[htb]
    \begin{center}
      \begin{tabular}{ | m{2cm} | m{2cm} | m{2cm} | m{2cm} | }
        \hline
      \multicolumn{1}{|c||}{\textbf{DEM}} & \multicolumn{1}{c|}{\textbf{DEM Resolution}} & \multicolumn{1}{c|}{\textbf{DEM Accuracy}} & \multicolumn{1}{c|}{\textbf{Area of missing data}} \\
        \hline\hline
          \multicolumn{1}{|c||}{GTOPO30~\cite{global30arc}} & \multicolumn{1}{c|}{900 mts} & \multicolumn{1}{c|}{30m} & \multicolumn{1}{c|}{None} \\
        \hline
          \multicolumn{1}{|c||}{NOAA Globe~\cite{hastings1993global}} & \multicolumn{1}{c|}{900 mts} & \multicolumn{1}{c|}{30m} & \multicolumn{1}{c|}{None} \\
        \hline
          \multicolumn{1}{|c||}{SRTM~\cite{jarvis2008hole}} & \multicolumn{1}{c|}{90 mts and 30 mts} & \multicolumn{1}{c|}{10m} & \multicolumn{1}{c|}{Topographically steep areas} \\  
        \hline
          \multicolumn{1}{|c||}{ASTER GDEM~\cite{paul2004combining}} & \multicolumn{1}{c|}{30 mts} & \multicolumn{1}{c|}{14 mts} & \multicolumn{1}{c|}{Areas with constant cloud cover} \\
        \hline
          \multicolumn{1}{|c||}{Lidar~\cite{gesch2009analysis}} & \multicolumn{1}{c|}{1 mts} & \multicolumn{1}{c|}{15 cm} & \multicolumn{1}{c|}{available at certain areas} \\
        \hline
      \end{tabular}
    \end{center}
    \caption{Various DEM services}
        \label{tab:DEM_services}
\end{table*}

From the table~\ref{tab:DEM_services}, we can see that DEMs GTOPO30 and NOAA GLOBE has poor resolution and accuracy. LIDAR has higher accuracy and resolution, but it’s just for specialized enterprise coverage specific to certain areas. So, the choice of SRTM data which have good accuracy and resolution is the best.



The data collected by SRTM has voids~\cite{robinson2014earthenv}. Two groups of scientists worked to fill the voids for different purposes, the CGIAR-CSI versions and the USGS HydroSHEDS dataset. The CGIAR-CSI version 4 provides the best global coverage for the full resolution SRTM dataset. The HydroSHEDS dataset was generated for hydrological applications and is suitable for consistent drainage and water flow information. In our investigation, we have used elevation information created by  Shuttle Radar Topography Mission (SRTM), which is provided by CGIAR-CSI. 

Using CGIAR-CSI GeoPortal, we can get the elevation data of terrain in the intervals of 5$^{\circ} \times 5^{\circ}$ tiles. The elevation produced by SRTM has a resolution of 90m at the equator. The elevation data are available in both ArcInfo ASCII and GeoTiff format~\cite{srtm_ascii_tiff}, which is easy to process for our purpose.

Figure~\ref{fig:srtm dataset} gives an illustration of a sample SRTM data points.

\begin{figure}[htb]
  \begin{center}
    \centering
    \includegraphics[scale=0.3]{./images/srtm_overlap.png}
    \caption{Information about dataset}
    \label{fig:srtm dataset}
  \end{center}
\end{figure}
The points along the same vertical line have the same longitude, but different latitudes differ by 0.000833 degrees. Similarly, the points along the same horizontal line have the same latitude, but different longitudes differ by 0.000833 degrees. 

Suppose we want the elevation at the Geo to co-ordinate $P(x, y)$, we can find the nearest data point $Q$ in the dataset and may assume $Q$'s elevation as $P$'s elevation. It will work well for city areas that are flat and have little elevations. However, it won't be accurate for mountainous roads. The elevation values differ a lot between two points on the stretch of road passing through mountains. So we need to generate a new data point using the dataset.

\subsubsection{Bilinear interpolation}

Generally, interpolation~\cite{davis1975interpolation} is used to find a new data point using the known data points. Fig~\ref{fig:illustration_interpolation} illustrates how interpolation is used.
\begin{figure}[htb]
  \begin{center}
    \includegraphics[scale=0.35]{./images/interpolate.jpg}
  \end{center}
    \caption{The four corners are the known data points and the point P at which we want to interpolate.}
    \label{fig:illustration_interpolation}
\end{figure}
Let the function $E:P\rightarrow R $, where $ R $ is the set of points on the real line, and $ P $ is at any point on the road. % represent the elevation values  $E(P)$ give the elevation of any general point $P$. 
Suppose, we know the values of set of four given points $A_{11}$, $A_{21}$, $A_{22}$, $A_{12}$. % $E(A_{11}), E(A_{21}), E(A_{22}), E(A_{12})$.
First, we need to carry out linear interpolation along the $X$-direction, that results:
$$ E(x, b_1) = \frac{a_2 - x}{a_2 - a_1} E(A_{11}) + \frac{x - a_1}{a_2 - a_1} E(A_{21}) $$
$$ E(x, b_2) = \frac{a_2 - x}{a_2 - a_1} E(A_{12}) + \frac{x - a_1}{a_2 - a_1} E(A_{22}) $$
Next, we need to perform linear interpolation along the $Y$-direction, that results:
$$ E(x, y) = \frac{b_2 - y}{b_2 - b_1} E(x, b_1) + \frac{y - b_1}{b_2 - b_1} E(x, b_2) $$
We can use non-linear interpolations also.

\subsubsection{Example}

Now let's consider following the mountainous road from Tirumala to Tirupati and compare the elevations along the path with naive, interpolation, and Google Maps data.
\begin{figure}[htb]
  \begin{center}
    \includegraphics[scale=0.25,angle=-90]{./images/tml_ghat.pdf}
  \end{center}
    \caption{A stretch of 260m on a mountainous road.}
    \label{fig:ghat_road}
\end{figure}
We first divide the path of 258m into seven segments. In the figure, the marker $A$ is the starting position and the marker $H$ is the final position. 
\begin{table*}[htb]
    \begin{center}
      \begin{tabular}{ | m{4cm} | m{4cm} | m{5cm} | m{5cm} | }
        \hline
      \multicolumn{1}{|c||}{ \textbf{\backslashbox{Position}{Elevation}} } & \multicolumn{1}{c|}{\textbf{Rounding of to \newline nearest point(m)}} & \multicolumn{1}{c|}{\textbf{Interpolation}} & \multicolumn{1}{c|}{\textbf{Google Maps}} \\
        \hline\hline
          \multicolumn{1}{|c||}{A} & \multicolumn{1}{c|}{817} & \multicolumn{1}{c|}{822.33} & \multicolumn{1}{c|}{821.5} \\
        \hline
          \multicolumn{1}{|c||}{B} & \multicolumn{1}{c|}{839} & \multicolumn{1}{c|}{815.27} & \multicolumn{1}{c|}{812.22} \\
        \hline
          \multicolumn{1}{|c||}{C} & \multicolumn{1}{c|}{789} & \multicolumn{1}{c|}{809.46} & \multicolumn{1}{c|}{806.35} \\
        \hline
          \multicolumn{1}{|c||}{D} & \multicolumn{1}{c|}{800} & \multicolumn{1}{c|}{804.802} & \multicolumn{1}{c|}{804.167} \\
        \hline
          \multicolumn{1}{|c||}{E} & \multicolumn{1}{c|}{800} & \multicolumn{1}{c|}{806.41} & \multicolumn{1}{c|}{805.41} \\
        \hline
          \multicolumn{1}{|c||}{F} & \multicolumn{1}{c|}{800} & \multicolumn{1}{c|}{811.72} & \multicolumn{1}{c|}{810.55} \\
        \hline
          \multicolumn{1}{|c||}{G} & \multicolumn{1}{c|}{827} & \multicolumn{1}{c|}{822.99} & \multicolumn{1}{c|}{822.4} \\
        \hline
          \multicolumn{1}{|c||}{H} & \multicolumn{1}{c|}{827} & \multicolumn{1}{c|}{827.79} & \multicolumn{1}{c|}{827.1} \\
        \hline
      \end{tabular}
    \end{center}
    \caption{Comparing SRTM results with Google Maps}
        \label{tab:srtm_gmap}
\end{table*}

The table~\ref{tab:srtm_gmap} have the comparison of the SRTM elevation data without interpolation, with interpolation and Google Map elevation. From this, we can observe that SRTM data with interpolation gives us good accuracy.
Now we can calculate elevation at any given Geo co-ordinate. Therefore, we can now calculate the gradient of a road segment easily. Depending on the gradient, we calculate Road Gradient Factor.
Once the gradient of the road is known, we can use Equation~\ref{eq:FC} to change the edge weights of the graph into fuel consumption. Therefore, we can find the least fuel path for a given source and a destination. The next section discusses the results.



==> sections/oldGMaps.tex <==
\section{Google Maps and Open Street Map}
\label{ch:gmap}
Developing an eco-friendly vehicle routing from scratch is not feasible without a large team working on it. Our aim is to assessing problems likely to appear in trying to enhance an  existing navigation tool for eco-friendliness. Therefore, we started by exploring the different APIs provided by Google Maps and Open Street Map for the purpose of navigation.   %Our first idea is to explore existing navigation tools and try incorporating a way to estimate fuel consumption depending on vehicle speeds. 
%The driver of the vehicle just inputs source and destination and would expect that the navigation tool will provide a route itinerant complete with an estimated fuel consumption. %ultimately and we will see how we use these to get our work done.

%\subsection{Different APIs}
\subsection{Geo-Coding}
We start with a precise definition of the problem. %statement. 
\begin{definition}[Problem statement] 
Given a source $S$ and a destination $B$, find the optimal fuel path.
\end{definition}
The first requirement is how to specify a source or a destination. From point of view of navigation, it would be the addresses the source and then destination. The format of an address should be in human understandable form, e.g., a street address.

Geo-coding is defined as the process of converting human readable street addresses into geographic coordinates. More precisely, each address is  converted into a (latitude, longitude) pair. The geographic coordinates are convenient as these can be used  to place the markers on a map and to find  the distance or elevation between a source and a destination. 

\subsection{Google Map APIs}
Google Maps API tool provides for extracting geo-coordinates for an address by using the following API:

\url{https://maps.googleapis.com/maps/api/geocode/json?address=<ADDRESS>&key=<KEY>}

Along with latitude and longitude coordinates, it also provides other address components such as state, country, pin code, etc.
For example, using the ADDRESS = "cse IIT Kanpur" returns Geo-coordinates (26.5143, 80.2348).

\subsubsection{Places Nearby}

Google API can be used to find important utility points near a pre-specified location. For example,  utility points of interest could be the nearby restaurants, car service stations, hospitals, fuel pumps, convenience stores, govt offices, etc. The API call given below extracts the location and other information about the nearby restaurants.  

\url{https://maps.googleapis.com/maps/api/place/nearbysearch/json?location=26.5143, 80.2348&rankby=distance&type=restaurant&key=<KEY>}\\
In the above example, it returns the restaurants details nearby given coordinates (CSE IIT Kanpur), sorted by the distance

\subsubsection{Elevation}

The elevation values represent the elevations relative to the sea level. For finding the elevation at some Geo coordinate, we use the following GoogleMap API.

\url{https://maps.googleapis.com/maps/api/elevation/json?locations=26.5143, 80.2348&key=<KEY>}\\
It returns the elevation at CSE IIT Kanpur.

\subsubsection{Direction}

A direction is represented as series of Geo coordinates along the path. To extract the series of Geo coordinates from a source to a destination we use the following GoogleMap API. We need to go via these Geo coordinates while driving.

\url{https://maps.googleapis.com/maps/api/directions/json?origin=<Geo Cordinates>&destination=<Geo Cordinates>&key=<KEY>}\\
This API returns polylines (a sequence of straight lines) from a source to a destination. This polyline contains encrypted geo coordinates. We need to decrypt them and extract a sequence of geo-coordinates from all those polylines.

Figure~\ref{fig:direction_gmap} shows the graphical display of the direction from CSE IIT Kanpur to Lucknow Airport.
\begin{figure*}
  \begin{center}
    \centering
    \includegraphics[scale=0.4]{./images/gmap_api/direction.png}
    \caption{Direction service provided by Google from CSE IIT Kanpur to Lucknow Airport}
    \label{fig:direction_gmap}
  \end{center}
\end{figure*}
%\clearpage

\subsubsection{Elevation Along a Path}
By using `getElevationAlongPath' API, We can find the elevation level along the path from a source to a destination. As shown in the Fig.~\ref{fig:elevation_path}, upper graph shows the elevations along the path from ‘CSE IIT Kanpur’ to ‘Lucknow Airport’.
\begin{figure*}
  \begin{center}
    \centering
    \includegraphics[scale=0.25]{./images/gmap_api/elevation_along_path.png}
    \caption{Elevation and normalized elevation along the path}
    \label{fig:elevation_path}
  \end{center}
\end{figure*}

To understand how the road is, we normalized the road elevations by talking the minimum raise/drop in the elevation between two consecutive points $\triangle$e=5m. The lower half of Fig~\ref{fig:elevation_path} gives the normalized elevations.

Using the direction service we can even find the distance and the time required to travel along the path. Therefore, it is possible to calculate the average velocity along the route. By using Elevation service we can calculate the road gradient along the road. Once road gradient is available the equation~\ref{eq:FC} can be used to find the fuel consumption for a given route.
\subsubsection{Fuel Estimation}
We built a simple application which uses the above APIs, and calculates Fuel consumption for the path provided by Google Maps. Fig.~\ref{fig:fuel_gmap_1} and~\ref{fig:fuel_gmap_2} provide screenshots of two different source-destination pairs obtained from our application.
\begin{figure*}
  \begin{center}
    \centering
    \includegraphics[scale=0.2]{./images/gmap_api/fuel_1.png}
    \caption{CSE IIT Kanpur to Lucknow airport}
    \label{fig:fuel_gmap_1}
  \end{center}
\end{figure*}

For a better visualization of the elevation of the along the road, we divided the road into intervals of 256km each. 
\begin{figure*}
  \begin{center}
    \centering
    \includegraphics[scale=0.25]{./images/gmap_api/fuel_2.png}
    \caption{IITK to Delhi}
    \label{fig:fuel_gmap_2}
  \end{center}
\end{figure*}
As shown in the Fig.~\ref{fig:fuel_gmap_2} we can observe that for the first 256km there is a 20m rise in elevation which requires a fuel consumption of 14.5 liters. However, for the next part 247km there is 65m rise in the elevation and the fuel consumption increase to 18.2 liters. We can clearly see the effect of the gradient.
\subsection{Limitations of Google Map API}
The limitations of Google Maps is that it only estimate the fuel consumption for the given routes. In other words, it is possible to calculate fuel consumption if we know the path. However, our aim is to estimate the least fuel consumption route. So the routing algorithm has to incorporate fuel requirement as a basis for finding the path and not the time or distance. Unfortunately, Google Maps don’t have any API which uses fuel consumption as a basis for route computation. Furthermore, we cannot apply our routing algorithms on the Google Maps because it does not provide us the raw data of the maps.

\section{Open Street Maps (OSM)}
Limitations of Google Map APIs forced us to search for the raw map data. We find projects regarding to collaborative mapping~\cite{goodchild2007citizens},where the users collect the data. The open source collaborative mapping called “Open Street Map” (OSM) which not only competes with commercial services like
Google Maps but also provides the raw map data. OSM data is entirely crowdsourced, and anyone can use/edit the map data~\cite{OSM} at free of cost.


Structurally, OSM consists of two different types of elements:
\begin{itemize}
    \item Node: It contains places defined with it’s Geo Coordinates
    \item Way: It contains the roads, boundaries of the building, places. For the roads, it’ll be having detail description of the road like name of the road, whether the road is motorway/trunk/residential etc.
\end{itemize}

There is a project called Open Source Routing Machine (OSRM). It is a Routing Engine which is basically an implementation of multi level Dijkstra’s shortest path algorithm on a graph built from the OSM data. The edge weights of the graph are distances or duration for covering those distances. Therefore, the routing based on the least distance or the least travel time. However, the good part of the implementation is that it possible to fix a velocity, depending on the type of the road. Table~\ref{tab:OSRM_velocity} gives a specification of those values.
\begin{table}[htb]
\begin{center}
  \begin{tabular}{ | m{5cm} | m{5cm} | }
    \hline
      \multicolumn{1}{|c|}{\textbf{Road Type}} & \multicolumn{1}{c|}{\textbf{velocity(km/hr)}} \\
    \hline\hline
      \multicolumn{1}{|c|}{motorway} & \multicolumn{1}{c|}{90} \\
    \hline
      \multicolumn{1}{|c|}{motorway\_link} & \multicolumn{1}{c|}{45} \\
    \hline
      \multicolumn{1}{|c|}{trunk} & \multicolumn{1}{c|}{85} \\
    \hline
      \multicolumn{1}{|c|}{trunk\_link} & \multicolumn{1}{c|}{40} \\
    \hline
      \multicolumn{1}{|c|}{primary} & \multicolumn{1}{c|}{65} \\
    \hline
      \multicolumn{1}{|c|}{primary\_link} & \multicolumn{1}{c|}{30} \\
    \hline
      \multicolumn{1}{|c|}{secondary} & \multicolumn{1}{c|}{55} \\
    \hline
      \multicolumn{1}{|c|}{secondary\_link} & \multicolumn{1}{c|}{25} \\
    \hline
      \multicolumn{1}{|c|}{tertiary} & \multicolumn{1}{c|}{40} \\
    \hline
      \multicolumn{1}{|c|}{tertiary\_link} & \multicolumn{1}{c|}{20} \\
    \hline
      \multicolumn{1}{|c|}{unclassified} & \multicolumn{1}{c|}{25} \\
    \hline
      \multicolumn{1}{|c|}{residential} & \multicolumn{1}{c|}{25} \\
    \hline
      \multicolumn{1}{|c|}{living\_street} & \multicolumn{1}{c|}{10} \\
    \hline
      \multicolumn{1}{|c|}{service} & \multicolumn{1}{c|}{15} \\
    \hline
  \end{tabular}
\end{center}
\caption{Velocity on various roads}
    \label{tab:OSRM_velocity}
\end{table}
Considering the fact that OSRM provides raw map data and the fact that it has a specification of vehicle velocity on the basis of road type, we decided to implement our project on Open Street Maps and OSRM. %we will be using OSRM to solve our problem of finding a route by considering fuel consumption factor.



==> sections/oldback.tex <==
\section{Background and Related Work}
\label{ch:bcg}

%{\color{red}{Comment: The chapter should also include related work}}

%Surface transportation system is critical to economic and social growth of human settlements across the globe. Therefore, it is important to invest time in planning and maintenance of the layout for transportation networks. The surface transportation system consists of roads, rail roads and shipping channels.
Our focus here is on road transportation system for vehicular movements which depend on burning of fossil fuel. Burning of fossil fuel causes harmful emissions which affects the environment adversely. Apart from just developing a good road infrastructure, we need sound methods to assess fuel consumption, emissions, and good strategies to reduce the adverse effects of emission on the environment. Therefore, eco-friendly routing for vehicular movements between a source destination pair is significant in the context of road navigation. Before addressing the problem, we need to understand the background about appropriate models that may used for estimation of emission and fuel consumption from different vehicle types. The concern here is to integrate both fuel consumption assessments and the road elevation data with widely use routing machines such as Google Maps or Open Street Maps to generate a eco-friendly route between a source and a destination. % with least fuel consumption along with an estimated time to the users. 

\subsection{Eco-friendly Routing}
Eco-routing solutions allow for the prediction of the most fuel-economic routes and are of interest to the transportation industry as they offer a way to reduce fuel consumption and emissions dramatically. However, there has been little development of tools in providing solutions to individuals which will create awareness about the impact of choosing an eco-friendly path. From the point of view of businesses, saving the fuel means saving money. 

Many factors affect a vehicle emissions and fuel consumption. However, three most important factors are vehicle characteristics, road characteristics, and traffic conditions. Each type of vehicle has different aerodynamic drags, different engine technology which determines its fuel efficiency.% The consumption of fuel varies with the type of vehicle, as  , and uses a specific fuel type.%, etc.
Fuel consumption and vehicle emissions are sensitive to changes in travel speed, traffic patterns, etc. A small portion of the route may account for substantial portion of total fuel consumption depending on traffic intensity~\cite{wang2019real}. The gradient of road plays another important role in understanding vehicle's fuel efficiency as real world fuel consumption and emission models are sensitive to road grade estimates. Some research~\cite{yao2013study} indicate that the road grade accounts for approximately 1-3\% of fuel consumption use in light duty vehicles.
The eco-friendly route will be the least fuel consumed route among all the possible routes for a given source and destination.
Therefore, the estimate of fuel consumption requires %So we need
the entire road curvature data for the complete path from source to destination. Finally, from the point of view of a driver of a vehicle, it is extremely convenient and a practical approach to embed a routing engine in existing navigation tools for the purpose of commutation and transportation. In summary,
finding eco-friendly routing between a source and a destination require three basic components:
\begin{itemize}
    \item A model for estimating emissions from different vehicle types and a compilation method for calculation of aggregated emission data under different road surfaces and traffic conditions.
    \item A road network database incorporating a digital road map with historical data together with data fusion strategies for integrating crowd sourced real-time traffic.
    \item A user interface for taking driver’s input and display the route on a road map, along with fuel consumed, and travel itinerary 
\end{itemize}

Thus, developing an eco-friendly navigation tool is far too a complex to build from scratch. It requires a sustained long term team effort which can only be possible by  Google, Microsoft, etc. Therefore, in this thesis we employed following short cuts:
\begin{enumerate}
    \item For road network databases we leveraged two well established navigation and route machines, namely, Google Maps~\cite{GoogleMaps} and Open Street Maps~\cite{OSM}.
    \item For estimating fuel consumption, we used HERA methodology~\cite{HERA2016}.
    \item  For display of maps and least fuel cost routes, we used a third party front end builder. % for OSM.
    \item For  compiling travel itinerary we used Google multipoint representation of turns, etc. 
    \item For integrating real time mobile navigation interface, we employed another third party application. 
\end{enumerate} 


\subsection{HERA Methodology}

Many models exist for estimation of emission due to road traffic and energy consumption.  We can analyze the traffic flows from two general perspectives,
\begin{enumerate}
    \item Microscopic.
    \item Macroscopic.
\end{enumerate} 
A Microscopic view of traffic takes into account the vehicle related variables and the traffic flow characteristics. The vehicle related variables are the length of the vehicle, the speed and the acceleration. The traffic flow characteristics refer to the variability in traffic stream which depend on both physical constraints and the complex behavior of drivers. The space gap between two vehicles, time variability between different traffic streams constitute to the variability in traffic stream. For macroscopic analysis of traffic instead of looking into each vehicle, we investigate on an aggregate picture of vehicular movements~\cite{trafficflow}.

Two prominent simulators widely used to model emission from vehicles are: 
\begin{itemize}
    \item The COPERT~\cite{COPERT2009} – COmputer Programme to calculate Emissions from Road Transport.
    \item  MOVES~\cite{MOVES2010} – Motor Vehicles Emission Simulator.
\end{itemize}
Both models use their own databases to obtain the emission factors as a function of average cycle of speeds. COPERT is mainly used in Europe while MOVES is used in the USA. There are other types of simulators which take microscopic details into account for measuring and calculating emission maps with speed and acceleration.

%The energy consumption and emission modeling tools provide quantitative evaluation of emission and provide quantitative ways to optimize emissions. 
The energy consumption and emission modeling tools provide quantitative evaluation for a given route.
For our  purposes, we have used models created based on HERA~\cite{HERA2016} methodology. It uses an average speed consumption model, based on COPERT emission factors.  These factors are adjusted with a correction factor to incorporate the gradient effect on the vehicles in each road section.\\

The average speed is a key factor in fuels consumption and emissions of vehicle. Several studies~\cite{HERA2016} have found that there is a relation between the fuel consumption and vehicle speed. Therefore, it is very appropriate to use the models which are based on speed. Since HERA consumption model is based on consumption and emission factors from COPERT, it considers a set of vehicle-centric parameters to calculate fuel consumption. For example in the case of light vehicle (passenger cars), it uses the fuel type and engine capacity and engine technology and for heavy vehicle it uses the maximum total weight, load state, the engine technology and the road gradient. %for heavy vehicles.
%For estimating the consumption and emission factors, COPERT \\

HERA~\cite{HERA2016} uses a slightly altered set of parameters. It take the average speed as the leading factor and the road gradient as a correction factor. It considers six vehicle types, namely,  passenger cars, light-duty vehicles, motorcycles, rigid trucks, articulated trucks, and buses.  HERA methodology provides an analytical formula to determine an approximates relationship between the fuel Consumption and the average speed for each category of vehicle. Table~\ref{tab:tab1background} summarizes the relationships.
\begin{table*}[htb]
\begin{center}
  \begin{tabular}{ | m{5cm} | m{5cm} | }
    \hline
      \multicolumn{1}{|c|}{\textbf{Vehicle Type}} & \multicolumn{1}{c|}{\textbf{Fuel Consumption Function for 0\% Road Gradient (gfuel/veh-km)}} \\
    \hline\hline
      \multicolumn{1}{|c|}{Motor Cycle} & \multicolumn{1}{c|}{25.722 + (276.13/V) + (-0.254)*V + 0.00311*V$^2$} \\
    \hline
      \multicolumn{1}{|c|}{Passenger Car} & \multicolumn{1}{c|}{54.7 + (496/V) + (-0.542)*V + 0.0042*V$^2$} \\
    \hline
      \multicolumn{1}{|c|}{Light-Duty Vehicle} & \multicolumn{1}{c|}{146.27 + ((-0.0000106)/V) + (-2.596)*V + 0.01984*V$^2$} \\
    \hline
      \multicolumn{1}{|c|}{Rigid Truck} & \multicolumn{1}{c|}{152.96 + (604.156/V) + (-2.295)*V + 0.0238*V$^2$} \\
    \hline
      \multicolumn{1}{|c|}{Articulated Truck} & \multicolumn{1}{c|}{332.603 + (1680.879/V) + (-4.676)*V + 0.0311*V$^2$} \\
    \hline
      \multicolumn{1}{|c|}{Bus} & \multicolumn{1}{c|}{281.735 + (4186.178/V) + (-3.457)*V + 0.0216*V$^2$} \\
    \hline
  \end{tabular}
\end{center}
\caption{Approximate relationships between speed and fuel consumption for each vehicle type.}
    \label{tab:tab1background}
\end{table*}
Overall Fuel Consumption, 
\[
     FC_i =  FCZ_i * RGF_i,
    \label{eq:FC}
\]
where $FCZ$ is the fuel consumption on road with zero gradient, $RGF$ is the Road Gradient Factor, and $i$ represent different type of vehicles car, bus, etc.

HERA uses the consumption factors of each vehicle category and consumption curves data from COPERT database to construct above formulae.  By applying the non-linear regression techniques and parametrization of the consumption curves HERA derives the consumption model function for each vehicle type, excluding the Road Gradient Factor RGF.

\subsection{Road Gradient Factor}

Apart from average vehicle speeds, there are many other parameters that affect fuel consumption. These include a wear-and-tear of vehicle, the technology used, and the state of the road, the elevation of the road (or Road Gradient), Road Surface.

The gradient of a road has the effect of increasing or decreasing the resistance of a vehicle to traction. The increase or decrease in the load on the engine have a corresponding effect on the rates of emission and the fuel consumption. The effect of road gradient on the vehicle is not symmetrical, i.e., the extra fuel consumed by traveling uphill won’t be equal to the reduced fuel consumption when traveling downhill. In general, the effect of road gradient is more on the lighter vehicle than on the heavy-duty vehicles.

For a given speed $V$, the fuel consumed on the flat road is different compared to either uphill or downhill. HERA uses a correction factor which is based on the results of the German Emission Factor Programme~\cite{de2004modelling}. Some of the factors included in the correction are:
\begin{enumerate}
  \item The road gradient
  \item The pollutant
  \item The average speed of the vehicle
  \item The vehicle category
\end{enumerate}
The road gradient factor $RGF_i$ for each vehicle type $i$ is found according to following formula:
\[
\begin{split}
RGF_i &= A6_{i,k} * V^6 + A5_{i,k} * V^5 + A4_{i,k} * V^4 + A3_{i,k} * V^3 \\
& + A2_{i,k} * V^2 + A1_{i,k} * V + A0, 
\end{split}
\]
where RGF$_i$ is the road gradient factor for the vehicle category $i$, $V$ is the average speed of the vehicle in km/hr. $A0$ to $A6$ are the coefficients depending on the gradient and the type of the vehicle provided by Hickman et al.~\cite{MEET1999}.

%Further, in this project, we will be using these equations to compute the fuel consumption along the route.

==> sections/oldofrm_result.tex <==
\section{Results and Analysis}
\label{ch:result}

%\{Input}
In this chapter we discuss the results from Optimal Fuel Routing Machine (OFRM). At present OFRM accepts Geo-coordinates or the addresses as source and destination. It allows a user also to select the places on the map by placing a marker for a source and another for a destination. 
OFRM displays a complete description of the route between a given source destination pair in terms of distance of each road segment, the associated directions and the turns required. It also displays three values, namely, the distance, the time and the fuel consumption needed to travel in that entire path. Some the screenshots from OFRM are given below for the reader to understand the advantage of navigational outputs from OFRM.

\begin{figure*}[H]
  \begin{center}
    \centering
    \includegraphics[width=1.0\textwidth , height=6.5cm]{./images/ofrm_img/iisc_to_majestic.png}
    \caption{IISC Bengaluru to Bengaluru Bus Station, input supplied as address}
    \label{fig:iisc_to_majestic_route}
  \end{center}
\end{figure*}

From Fig~\ref{fig:iisc_to_majestic_route}, we can observe that there is small box on the top left where the user specifies inputs for the source and the destination. A graphical display of the route between src to dst appears marked in thick blue. In the right part of the display window, the details of travel itinerary are provided with exact navigational instructions for distance to be traveled for a segment of road and the type of turns (left, right or u-turns) to be executed. % needs to take like Right Turn or Left Turn or U-Turn.
To show the map tiles we used Mapbox APIs~\cite{mapbox}, for the detailed travelling itinerary we used leaflet library~\cite{leaflet}.

Our system also allows the user to select the source and the destination on the map instead of providing the address in the input. The markers are associated with (lat, long) pairs. So, the marker-based inputs will be interpreted as Geo-coordinates for the routing engine. The user also has an option to supply the input directly as Geo-coordinates.

\begin{figure*}[H]
  \begin{center}
    \centering
    \includegraphics[width=1.0\textwidth , height=15cm]{./images/ofrm_img/kia_to_iisc.png}
    \caption{Bengaluru Airport to IISC Bengaluru, selecting inputs on the map}
    \label{fig:kia_to_iisc}
  \end{center}
\end{figure*}

Fig~\ref{fig:kia_to_iisc} illustrates an example, where the user selected the source as Bengaluru's International Airport and the destination as IISC on the map. So, the input is treated as Geo-coordinates. As a result we can see the graphical route and travel itinerary between the source and destination.
%\clearpage

If a user wants to find a route that goes via some chosen places, then it is possible to request the routing engine to display a least fuel cost path by specifying any finite number of way points.
\begin{figure*}[H]
  \begin{center}
    \centering
    \includegraphics[width=1.0\textwidth , height=15cm]{./images/ofrm_img/kia_whitefield_iisc.png}
    \caption{Bengaluru Airport to IISC Bengaluru via Whitefield}
    \label{fig:kia_whitefield_iisc}
  \end{center}
\end{figure*}

For example, suppose a user wants to travel from source (airport) to the destination(IISC) via whitefield. Then user gives the three inputs, the source, the destination and the way point. The routing engine will give route from airport to IISC via whitefield, which we can see in the Fig~\ref{fig:kia_whitefield_iisc}.
%\clearpage

\subsubsection*{Comparing mountainous Roads}

In the next section we indicate how the gradient of the road effects the fuel consumption. For this we selected some of the mountainous roads, namely,  Tirupati-Tirumala, Aluva-Munnar, Kullu-Manali and Kalka-shimla.

For each road we compared the duration of the travel from Google Maps, the output from OFRM (our routing engine) without considering the Road Gradient then the output of OFRM taking the gradient of the road from SRTM dataFactor. %So, for computation of OFRM output first RGF=1 and  the Equation~\ref{eq:FC} RGF = 1 and our routing engine .

\begin{table*}[htb]
  \begin{center}
    \begin{tabular}{ | m{3cm} | m{3cm} | m{3cm} | m{3cm} | m{3cm} | }
     \hline
       one-way Rd & \multicolumn{1}{c|}{\textbf{Elevation}} & \multicolumn{1}{c|}{\textbf{Google Maps}} & \multicolumn{1}{c|}{\textbf{OFRM-Zero}} & \multicolumn{1}{c|}{\textbf{OFRM-Gradient}} \\
     \hline\hline
      \href{https://www.google.com/maps/dir/13.647243,79.4056888/13.6723405,79.351532/@13.6560224,79.3556799,14z/data=!3m1!4b1!4m6!4m5!2m3!6e0!7e2!8j1558402200!3e0}{Tirumala Up Rd - 17km} & \multicolumn{1}{c|}{710m gain} & \multicolumn{1}{c|}{32min}  & \multicolumn{1}{c|}{16min, 1.03 Litres} & \multicolumn{1}{c|}{29min, 1.58 Litres} \\
     \hline
      \href{https://www.google.com/maps/dir/13.6723405,79.351532/13.647243,79.4056888/@13.6598245,79.3684709,14z/data=!3m1!4b1!4m6!4m5!2m3!6e0!7e2!8j1558402200!3e0}{Tirumala Down Rd - 17km} & \multicolumn{1}{c|}{710m drop} & \multicolumn{1}{c|}{37min}  & \multicolumn{1}{c|}{21min, 1.13 Litres} & \multicolumn{1}{c|}{38min, 1.07 Litres} \\
    \hline
    \end{tabular}
    \end{center}
    
    \begin{center}
    \begin{tabular}{ | m{3cm} | m{3cm} | m{3cm} | m{3cm} | m{3cm} | }
     \hline
       two-way Rd & \multicolumn{1}{c|}{\textbf{Elevation}} & \multicolumn{1}{c|}{\textbf{Google Maps}} & \multicolumn{1}{c|}{\textbf{OFRM-Zero}} & \multicolumn{1}{c|}{\textbf{OFRM-Gradient}} \\
     \hline\hline
       \href{https://www.google.com/maps/dir/10.0450775,77.0486689/10.1525203,77.0764999/@10.0988009,77.0454722,13.25z/data=!4m6!4m5!2m3!6e0!7e2!8j1558323000!3e0}{Aluva - Munnar Rd 18km} & \multicolumn{1}{c|}{570m gain} & \multicolumn{1}{c|}{40min}  & \multicolumn{1}{c|}{29min, 1.31 Litres} & \multicolumn{1}{c|}{51min, 1.94 Litres} \\
     \hline
      Aluva - Munnar Rd 18km & \multicolumn{1}{c|}{570m drop} & \multicolumn{1}{c|}{40min}  & \multicolumn{1}{c|}{29min, 1.31 Litres} & \multicolumn{1}{c|}{51min, 1.94 Litres} \\
    \hline
    \end{tabular}
    \end{center}
    
    \begin{center}
    \begin{tabular}{ | m{3cm} | m{3cm} | m{3cm} | m{3cm} | m{3cm} | }
     \hline
       two-way Rd & \multicolumn{1}{c|}{\textbf{Elevation}} & \multicolumn{1}{c|}{\textbf{Google Maps}} & \multicolumn{1}{c|}{\textbf{OFRM-Zero}} & \multicolumn{1}{c|}{\textbf{OFRM-Gradient}} \\
     \hline\hline
        \href{https://www.google.com/maps/dir/31.9607863,77.1147839/32.2371711,77.1867908/@32.1033314,77.0623144,11.5z/data=!4m2!4m1!3e0}{Kullu to Manali Rd - 38km} & \multicolumn{1}{c|}{680m gain} & \multicolumn{1}{c|}{1hr7min}  & \multicolumn{1}{c|}{29min, 2.33 Litres} & \multicolumn{1}{c|}{43min, 2.85 Litres} \\
     \hline
       Manali to Kullu Rd - 38km & \multicolumn{1}{c|}{680m drop} & \multicolumn{1}{c|}{1hr05min}  & \multicolumn{1}{c|}{29min, 2.33 Litres} & \multicolumn{1}{c|}{43min, 2.85 Litres} \\
    \hline
    \end{tabular}
    \end{center}
    
    \begin{center}
    \begin{tabular}{ | m{3cm} | m{3cm} | m{3cm} | m{3cm} | m{3cm} | }
     \hline
       two-way Rd & \multicolumn{1}{c|}{\textbf{Elevation}} & \multicolumn{1}{c|}{\textbf{Google Maps}} & \multicolumn{1}{c|}{\textbf{OFRM-Zero}} & \multicolumn{1}{c|}{\textbf{OFRM-Gradient}} \\
     \hline\hline
       \href{https://www.google.com/maps/dir/31.0928073,77.1366113/30.9692217,77.1055441/@31.0311885,77.0792033,13z/data=!3m1!4b1!4m2!4m1!3e0}{Kalka - Shimla Rd - 25km} & \multicolumn{1}{c|}{520m gain} & \multicolumn{1}{c|}{40min}  & \multicolumn{1}{c|}{18min, 1.51 Litres} & \multicolumn{1}{c|}{36min, 1.84 Litres} \\
     \hline
      Kalka - Shimla Rd - 25km & \multicolumn{1}{c|}{520m drop} & \multicolumn{1}{c|}{40min}  & \multicolumn{1}{c|}{18min, 1.51 Litres} & \multicolumn{1}{c|}{36min, 1.84 Litres} \\
    \hline
    \end{tabular}
  \end{center}
  \caption{Comparision of several mountainous roads using Google Maps, our routing engine with and  without considering the gradient}
  \label{tab:mountainous_roads}
\end{table*}
The different columns of Table~\ref{tab:mountainous_roads} represent the following values:
\begin{enumerate}
\item \textbf{Google Maps} - it gives the output from the routing engine of Google Maps. It gives the travel time without considering the traffic.
\item \textbf{OFRM-Zero} - it gives two outputs time and fuel consumed as estimated by the proposed routing engine without considering the gradient of the road.
\item \textbf{OFRM-Gradient} - it also gives two outputs time and the amount of fuel spent as estimated by the proposed routing engine when the road gradient is also considered. 
\end{enumerate}
From the Table~\ref{tab:mountainous_roads} we observe that output produced by \textit{OFRM-Gradient} appear more realistic in terms of the duration of travel time as well as the estimation of fuel consumption. Since the road gradient either ascent or descent slows down the vehicle speed and increases the total duration of travel time compared to the corresponding outputs obtained from {\em OFRM-zero}. %by  is more than the \textit{OFRM-zero} which in turn effects the fuel consumption, from this we can infer that gradient plays a big role in affecting fuel consumption.

\section{Considering the traffic}

Until now, we have chosen the vehicle velocity from Table~\ref{tab:OSRM_velocity} for the calculation of fuel consumption. The table specifies that the velocity is only dependent on the type of road. In other words, we used a set time invariant values for a vehicle's velocity. However, in a real-world scenario, human activities vary throughout the day and traffic pattern also varies accordingly. So choosing a constant velocity results in either underestimating or overestimating the fuel consumption. %values.

Choosing an appropriate value for the velocity is an important factor for computing fuel consumption. So we need to understand the trend of traffic flows throughout the day and obtain a dynamic set of velocity coefficients  for the velocities for the road types from Table~\ref{tab:OSRM_velocity}. In other words, by determining velocity coefficients it is possible to capture the dynamicity of the traffic conditions.  We approached the problem as follows in order to search for the appropriate velocity coefficients. We generated hundreds of source-destination pairs for different locations in five different cities across in India. Then using Google Map API, we determined the duration of travel  for each pair of source-destination on a weekday at different times of the day.
\begin{figure*}[H]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{images/traffic/bengaluru.png}
  \label{fig:traffic_blore}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{images/traffic/delhi.png}
  \label{fig:traffic_delhi}
\end{subfigure}

\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{images/traffic/hyderabad.png}
  \label{fig:traffic_hyd}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{images/traffic/kolkata.png}
  \label{fig:traffic_kolkata}
\end{subfigure}

\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{images/traffic/mumbai.png}
  \label{fig:traffic_mumbai}
\end{subfigure}%
\caption{Analyzing traffic in several cities at various times.}
\label{fig:cities_traffic}
\end{figure*}

We compared the travel times between source-destination pairs at 9AM, 5PM, and 11PM with corresponding the travel time at 3AM using. The rationale behind using 9AM and 5PM for the analysis of the travel data is explained by the fact that at these times of the day the vehicular movements reach peaks in almost all cities every where. At 11PM, traffic is related to the night life offered by the corresponding cities, but the traffic is expected to be relatively low compared to 9AM or 5PM. We have taken 3AM outputs as the reference because very little vehicular movements is expected around the time as it coincides with the normal cycle of human non-activity. Therefore, 3AM is treated as zero traffic time. %After generating travel times for different samples of source-destination pairs at three different times (9AM, 5PM, and 11PM) of the day,  we correlate them with travel times at 3AM. 
The values are tabulated in Table~\ref{tab:deviation_various_times}, where
t$_X$ represents the average time taken to travel 1km distance at "$X$:00" hours for $X \in \{3,9,17,23\}$.

\begin{table*}[htb]
    \begin{center}
      \begin{tabular}{ | m{5cm} | m{5cm} | m{5cm} | m{5cm} | }
        \hline
      \multicolumn{1}{|c||}{\textbf{city}} & \multicolumn{1}{c|}{\textbf{$\frac{t_9 - t_3}{t_3}$ }} & \multicolumn{1}{c|}{\textbf{$\frac{t_{17} - t_3}{t_3}$}} & \multicolumn{1}{c|}{\textbf{$\frac{t_{23} - t_3}{t_3}$}} \\
        \hline\hline
          \multicolumn{1}{|c||}{Bangaluru} & \multicolumn{1}{c|}{0.846 $\pm$ 0.232} & \multicolumn{1}{c|}{0.934 $\pm$ 0.213} & \multicolumn{1}{c|}{0.240 $\pm$ 0.035} \\
        \hline
            \multicolumn{1}{|c||}{Delhi} & \multicolumn{1}{c|}{0.698 $\pm$ 0.169} & \multicolumn{1}{c|}{0.670 $\pm$ 0.160} & \multicolumn{1}{c|}{0.242 $\pm$ 0.035} \\
        \hline
            \multicolumn{1}{|c||}{Hyderabad} & \multicolumn{1}{c|}{0.566 $\pm$ 0.153} & \multicolumn{1}{c|}{0.745 $\pm$ 0.148} & \multicolumn{1}{c|}{0.272 $\pm$ 0.055} \\
        \hline
            \multicolumn{1}{|c||}{Kolkata} & \multicolumn{1}{c|}{0.588 $\pm$ 0.140} & \multicolumn{1}{c|}{0.627 $\pm$ 0.193} & \multicolumn{1}{c|}{0.252 $\pm$ 0.042} \\
        \hline
            \multicolumn{1}{|c||}{Mumbai} & \multicolumn{1}{c|}{0.736 $\pm$ 0.278} & \multicolumn{1}{c|}{0.832 $\pm$ 0.170} & \multicolumn{1}{c|}{0.258 $\pm$ 0.044} \\
        \hline
      \end{tabular}
    \end{center}
    \caption{Additional time taken to travel 1km at different times of the day w.r.t 3AM.}
        \label{tab:deviation_various_times}
\end{table*}

From Table~\ref{tab:deviation_various_times}, we find that for travel in Bangaluru city:
\begin{itemize}
    \item At 9AM on an average it takes an extra time of (0.846 $\pm$ 0.232)t$_3$ mins to travel 1km distance,
    \item At 5PM on an average it takes an extra duration of (0.934 $\pm$ 0.213)t$_3$ mins, and
    \item At 11PM on an average it takes an extra duration of (0.240 $\pm$ 0.035)t$_3$ mins.
\end{itemize}
Similarly, we can infer the factors for additional time requirements to account for the nature of traffic in the other cities, namely Mumbai, Kolkata Delhi and Hyderabad. 

%When we tested our routing engine which uses Table~\ref{tab:OSRM_velocity} with the Google Map data at 9 AM, the deviation in Bengaluru is -42.3\%, it’s -46.7\% in Delhi. As it is deviating wildly because we can’t use the same speed as mentioned in Table~\ref{tab:OSRM_velocity} because of traffic. So we changed the velocity on various roads to Table~\ref{tab:OFRM_velocity_traffic}

To test accuracy of the proposed routing engine, we have compared its outputs for a set of sources-destination pairs with that of the Google Maps API when traveled around 9AM, and we computed the ratio (average time provided by OFRM/average time provided by Google API). For Bangluru, the value of the ratio is  0.577 and it is 0.533 for Delhi. The reason for the huge deviation with respect to Google Maps is  attributed to the static velocity values used by OFRM without reference to variation in time of the day. Since Google Maps collects live data its outputs are different from the outputs of our routing engine which uses velocity values from the static Table~\ref{tab:OSRM_velocity}. It implies that one single static velocity table for all cities and for all traffic trends cannot provide any meaningful output.
So, we have to choose different set of velocity values for 9AM. Using statistics of average values from Table~\ref{tab:deviation_various_times}, we find that the average velocity of the vehicle at 3AM is almost twice compared to the velocity of the vehicle at 9AM. Using this relation we can generate velocity Table~\ref{tab:OFRM_velocity_traffic} for different roads for 9 AM, by taking Table~\ref{tab:OSRM_velocity} as reference.
%\clearpage
\begin{table}[htb]
\begin{center}
  \begin{tabular}{ | m{5cm} | m{5cm} | }
    \hline
      \multicolumn{1}{|c|}{\textbf{Road Type}} & \multicolumn{1}{c|}{\textbf{velocity(km/hr)}} \\
    \hline\hline
      \multicolumn{1}{|c|}{motorway} & \multicolumn{1}{c|}{45} \\
    \hline
      \multicolumn{1}{|c|}{motorway\_link} & \multicolumn{1}{c|}{22.5} \\
    \hline
      \multicolumn{1}{|c|}{trunk} & \multicolumn{1}{c|}{42.5} \\
    \hline
      \multicolumn{1}{|c|}{trunk\_link} & \multicolumn{1}{c|}{20} \\
    \hline
      \multicolumn{1}{|c|}{primary} & \multicolumn{1}{c|}{32.5} \\
    \hline
      \multicolumn{1}{|c|}{primary\_link} & \multicolumn{1}{c|}{15} \\
    \hline
      \multicolumn{1}{|c|}{secondary} & \multicolumn{1}{c|}{27.5} \\
    \hline
      \multicolumn{1}{|c|}{secondary\_link} & \multicolumn{1}{c|}{12.5} \\
    \hline
      \multicolumn{1}{|c|}{tertiary} & \multicolumn{1}{c|}{20} \\
    \hline
      \multicolumn{1}{|c|}{tertiary\_link} & \multicolumn{1}{c|}{10} \\
    \hline
      \multicolumn{1}{|c|}{unclassified} & \multicolumn{1}{c|}{12.5} \\
    \hline
      \multicolumn{1}{|c|}{residential} & \multicolumn{1}{c|}{12.5} \\
    \hline
      \multicolumn{1}{|c|}{living\_street} & \multicolumn{1}{c|}{5} \\
    \hline
      \multicolumn{1}{|c|}{service} & \multicolumn{1}{c|}{7.5} \\
    \hline
  \end{tabular}
\end{center}
\caption{Velocity on various roads.}
    \label{tab:OFRM_velocity_traffic}
\end{table}


%when we tested our routing engine which uses updated Table~\ref{tab:OFRM_velocity_traffic} with the Google Map data at 9 AM, the deviation in Bengaluru reduced to  11.4\%, and to  5.9\% in Delhi.

When we reevaluated our routing engine which uses velocity Table~\ref{tab:OFRM_velocity_traffic} with the Google Map at 9AM, the ratio (average time provided by OFRM/average time provided by Google API) in Bangluru increased to 0.886  and in Delhi it increased to 0.941. 
So it is essential to generate velocity values for more time intervals for  different cities. These velocity values can be used by OFRM to produce results specific to the city’s traffic trends. 
%\clearpage

\section{Mobile Application}

We designed a mobile application using open source project osmbonuspack~\cite{osmbonus}, where the user can supply a source and a destination. The application sends a request to OFRM routing engine and using the response from OFRM, the application gives a graphical displays the least fuel route between the source and the destination along with the itinerary. 

The application can take the current location of the user from device's GPS chip as input. In this case the user don't need to provide a source. The application displays a marker at the current location of the user, as he changes the location the marker location in map also changes correspondingly. But we maintained the display of the route from his/her position to the destination. If user goes outside the route which routing engine provided the mobile application  sends a new request with the user's current position and gets corresponding route update. %the route correspondingly.
\begin{figure}[H]
        \centering
        \begin{minipage}[b]{0.25\textwidth}
            \centering
            \includegraphics[scale=0.09]{images/mobile_app/1.png}\\
            (a) Route from current location
           % \label{fig:app_route} 
        \end{minipage}\begin{minipage}[b]{0.25\textwidth}
                \centering
                \includegraphics[scale=0.09]{images/mobile_app/4.png}\\
                (b) Travel itinerary
                %\label{fig:app_itinerary}
        \end{minipage}
        \caption{Route and travel itinerary from current location of the user to destination.}
    \label{fig:ss_14}
\end{figure}
Figure~\ref{fig:ss_14} illustrate an example with GPS input.
On the left of the figure we can see the source as "My position", which is CSE Department and Destination as Lucknow Airport, we can see graphical route between source and destination, and also overall distance, duration and fuel required. In the right we have detailed travel itinerary.
\begin{figure}[H]
\begin{center}
 \begin{minipage}[b]{0.25\textwidth}
 \centering
  \includegraphics[scale=0.09]{images/mobile_app/2.png}\\
  (a) Current route.
  \end{minipage}\begin{minipage}[b]{0.25\textwidth}
  \centering
  \includegraphics[scale=0.09]{images/mobile_app/3.png}\\
  (b) Updated route.
  \end{minipage}
\end{center}
%  \caption{Route at current location}
 % \label{fig:cloc}
%  \end{subfigure}
 % \begin{subfigure}[b]{0.45\textwidth}
   
%    \caption{Route update with location change}
%    \label{fig:zoom_in}
%  \end{subfigure}
    \caption{As the current location changes the route gets updated.}
    \label{fig:ss_23}
\end{figure} 
Fig~\ref{fig:ss_23} illustrates the route update when the user moved away from the current route.  We can see the route from the current location of user (CSE Department) as the new route gets updated.





